Bounds on the lattice point enumerator via slices and projections

Gardner, Gronchi and Zong posed the problem to find a discrete analogue of M. Meyer's inequality bounding the volume of a convex body from below by the geometric mean of the volumes of its slices with the coordinate hyperplanes. Motivated by this problem, for which we provide a first general bound, we study in a more general context the question to bound the number of lattice points of a convex body in terms of slices as well as projections.

==> default_preamble.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}

\usepackage{graphicx}
\usepackage{subcaption}

\usepackage{xcolor}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\posint}{\mathbb{Z}_{>0}}

\newcommand{\K}{\mathcal{K}}
\newcommand{\Ko}{\mathcal{K}_o}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\spann}{\mathrm{span}}

\newcommand{\bd}{\mathrm{bd}}
\newcommand{\inter}{\mathrm{int}}
\newcommand{\cl}{\mathrm{cl}}
\newcommand{\vol}{\mathrm{vol}}


%boldsymbols for vectors
\newcommand{\vk}{{\boldsymbol k}}
\newcommand{\va}{{\boldsymbol a}}
\newcommand{\vb}{{\boldsymbol b}}
\newcommand{\vc}{{\boldsymbol c}}
\newcommand{\vd}{{\boldsymbol d}}
\newcommand{\ve}{{\boldsymbol e}}
\newcommand{\vf}{{\boldsymbol f}}
\newcommand{\vs}{{\boldsymbol s}}
\newcommand{\vt}{{\boldsymbol t}}
\newcommand{\vl}{{\boldsymbol l}}
\newcommand{\vu}{{\boldsymbol u}}
\newcommand{\vv}{{\boldsymbol v}}
\newcommand{\vw}{{\boldsymbol w}}
\newcommand{\vx}{{\boldsymbol x}}
\newcommand{\vy}{{\boldsymbol y}}
\newcommand{\vz}{{\boldsymbol z}}
\newcommand{\vh}{{\boldsymbol h}}
\newcommand{\vg}{{\boldsymbol g}}
\newcommand{\vm}{{\boldsymbol m}}
\newcommand{\vone}{{\boldsymbol 1}}
\newcommand{\vlambda}{{\boldsymbol \lambda}}
\newcommand{\vnull}{{\boldsymbol 0}}
\newcommand{\vq}{{\boldsymbol q}}
\newcommand{\vgamma}{{\pmb\gamma}}

%lattice points
\newcommand{\LE}{\mathrm{G}}
